CryptoVampire: Automated Reasoning for the Complete Symbolic Attacker Cryptographic Model

Cryptographic protocols are hard to design and prove correct, as witnessed by the ever-growing list of attacks even on protocol standards. Symbolic models of cryptography enable automated formal security proofs of such protocols against an idealized model, which abstracts away from the algebraic properties of cryptographic schemes and thus misses attacks. Computational models yield rigorous guarantees but support at present only interactive proofs and/or restricted classes of protocols. A promising approach is given by the computationally complete symbolic attacker (CCSA), formalized in the BC Logic, which aims at bridging and getting the best of the two worlds, obtaining cryptographic guarantees by symbolic analysis. The BC Logic is supported by a recently developed interactive theorem prover, Squirrel, which enables machine-checked interactive security proofs, as opposed to automated ones, thus requiring expert knowledge. We introduce the CryptoVampire cryptographic protocol verifier, which for the first time fully automates proofs of trace properties in the BC Logic. The key technical contribution is a first-order (FO) formalization of protocol properties with tailored handling of subterm relations. We overcome the burden of interactive proving in higher-order (HO) logic and automatically establish soundness of cryptographic protocols using only FO reasoning. On the theoretical side, we restrict full FO logic with cryptographic axioms to ensure that, by losing the expressivity of the HO BC Logic, we do not lose soundness. On the practical side, CryptoVampire integrates dedicated proof techniques using FO saturation algorithms and heuristics, which enable leveraging the state-of-the-art Vampire FO theorem prover as the underlying proving engine. Our experimental results show CryptoVampire's effectiveness of as a standalone verifier and in terms of automation support for Squirrel.

==> 101-figures/002-squirrel-grammar.tex <==
\begin{align*}
    I \coloneqq&\quad i \gsep \pmb{i}\\
    T \coloneqq&\quad		%\mathsf{init}
                \tau
				 \gsep\mathsf{a}\mleft[ \vec I \mright]
				\\%\gsep \mathsf{pred}(T)\\
    t \coloneqq&\quad	x
                \gsep \mathsf{n}\mleft[ \vec I \mright]
				\gsep f\mleft( \vec t \mright)
				%\gsep \mathsf{c}\mleft[ \vec \imath \mright] \mat T
				\gsep \mathsf{att}(t)
				\gsep \mmacro{input}{T}
				\gsep \mmacro{output}{T}
				\gsep \mmacro{frame}{T}\\
		& |\quad \textsc{if } \phi \textsc{ then } t \textsc{ else } t' \\
		%  \gsep %\textsf{if } \phi \textsf{ then } t \textsf{ else } t'
				% \gsep \textsf{find } i_1,\dots,i_l \textsf{ such that } \phi \textsf{ then } t \textsf{ else } t'\\
		& |\quad \mfindst{\vec I}{\phi}{t}{t'}\\
    A \coloneqq&\quad 		f\mleft( \vec t \mright)
				\gsep t \equiv t'
				\gsep i = i'
				\gsep T = T'
				\gsep T < T'\\
			& |\quad \mathsf{happens}(T)
				\gsep \mmacro{cond}{T}
				\gsep \mmacro{exec}{T} \\
    \phi \coloneqq&\quad 	x
                \gsep A
				\gsep \btop
				\gsep \bbot
				\gsep \phi \bwedge \phi'
				\gsep \phi \bvee \phi'
				\gsep \phi \bimplies \phi'
				\gsep \bneg \phi \\
		& |\quad \bforall i. \phi
				\gsep \bexists i. \phi
				\gsep \bforall \tau. \phi
				\gsep \bexists \tau. \phi
\end{align*}

where $f\in\mathcal{F}$, $\mathsf{n}\in \mathcal{N}$, %$\mathsf{c}\in \mathcal{C}$
and $\mathsf{a}\in \mathcal{A}$.

==> 101-figures/003-squirrel-macros.tex <==
\begin{mathpar}
    \textsf{cond}_0, \textsf{exec}_0 \mexpandto \btop

    \textsf{input}_0 \mexpandto \varnothing

    \textsf{frame}_0 \mexpandto \mmsg[\museminipage]{\textsf{init}}

    \textsf{cond}_\textsf{a}\mexpandto \mcond[\museminipage]{\sigmT^{-1}\left( \textsf{a} \right)}

    \textsf{output}_{\textsf{a}}\mexpandto \mmsg[\museminipage]{\sigmT^{-1}\left( \textsf{a} \right)}

    \textsf{exec}_{\textsf{a}}\mexpandto \textsf{cond}_{\textsf{a}} \bwedge \textsf{exec}_{\textsf{a}-1}

    \textsf{input}_{\textsf{a}}\mexpandto \textsf{att}\mleft( \textsf{frame}_{\textsf{a}-1} \mright)%\\

    \textsf{frame}_{\textsf{a}} \mexpandto \begin{minipage}{0.7\columnwidth}%
        \vspace{-5mm}\begin{multline*}\big< \textsf{exec}_{\textsf{a}}; \\
            \big< \textsc{if }\textsf{exec}_{\textsf{a}}
                \textsc{ then }\textsf{output}_{\textsf{a}}
                \textsc{ else }\textsf{err}; \\
                \textsf{frame}_{\textsf{a}-1}\big>\big>
        \end{multline*}
    \end{minipage}\vspace*{-5mm}
\end{mathpar}

==> 101-figures/007-full-grammar-2.tex <==
\begin{align*}
    I \coloneqq&\quad       i \gsep \pmb{i} &\text{of sort \idxt}\\
    N \coloneqq&\quad       \mathsf{n}\mleft[ \vec{I} \mright]
                                    &\text{of sort \noncet}\\
    T \coloneqq&\quad		\tau %\mathsf{init}
                                \gsep \mathsf{a}\mleft[ \vec{I}\mright]
                                    &\text{of sort \tpt}\\
                                    % \gsep \mathsf{pred}(T)\\
    t \coloneqq&\quad		x \gsep \bar{N}
                                \gsep f\mleft( \vec t \mright)
                                % \gsep \mathsf{c}\mleft[ \vec \imath \mright] \mat T
                                \gsep \mmacro{input}{T}
                                \gsep \textsc{if } \phi \textsc{ then } t \textsc{ else } t'
                                \gsep \mfindst{\vec\imath}{\phi}{t}{t'}
                                    & \text{of sort \msgt{}}\\
    \phi \coloneqq&\quad 	    x \gsep t \equiv t'
                                \gsep f\mleft( \vec t \mright)
                                \gsep \btop
                                \gsep \bbot
                                \gsep \phi \bwedge \phi'
                                \gsep \phi \bvee \phi'
                                \gsep \phi \bimplies \phi'
                                \gsep \bneg \phi
                                \gsep \bforall i. \phi
                                \gsep \bexists i. \phi
                                \gsep \bforall \tau. \phi
                                \gsep \bexists \tau. \phi
                                    &\text{of sort \condt}\\
    B \coloneqq&\quad       \meval{t}
                                \gsep \meval{f}( \vec B)
                                    &\text{of sort \bitstrt}\\
    A \coloneqq&\quad 		t = t'
                                \gsep B = B'
                                \gsep i = i'
                                \gsep T = T'
                                \gsep T < T'
                                \gsep \mathsf{happens}(T)
                                    & \text{of sort \boolt}\\
    S \coloneqq&\quad           t \sqsubseteq_* t'
                                \gsep t \sqsubseteq_* \phi
                                \gsep N \sqsubseteq_* t
                                \gsep N \sqsubseteq_* \phi
                                    & \text{of sort \boolt}\\
    \varphi \coloneqq &\quad           S
                                \gsep A
                                \gsep \meval{\phi}\top
                                \gsep \bot
                                \gsep \varphi \vee \varphi'
                                \gsep \varphi \wedge \varphi'
                                \gsep \varphi \Rightarrow \varphi'
                                \gsep \neg \varphi
                                \gsep \exists x. \varphi
                                \gsep \forall x. \varphi
                                    & \text{of sort \boolt}
\end{align*}

Where $f\in\mathcal{F}$, $\mathsf{n}\in \mathcal{N}$ and $\mathsf{a}\in \mathcal{A}$.

==> 101-figures/008-final-sq-macros.tex <==
\begin{mathpar}
    \textsf{cond}_0, \textsf{exec}_0 \mexpandto \btop

    \textsf{input}_0 \mexpandto \varnothing

    \textsf{frame}_0 \mexpandto \mmsg[\museminipage]{\textsf{init}}

    \textsf{cond}_\textsf{a}\mexpandto \mcond[\museminipage]{\sigmT^{-1}\left( \textsf{a} \right)}

    \textsf{output}_{\textsf{a}}\mexpandto \mmsg[\museminipage]{\sigmT^{-1}\left( \textsf{a} \right)}

    \textsf{exec}_{\textsf{a}}\mexpandto \textsf{cond}_{\textsf{a}} \mathbin{\dot{\wedge}} \textsf{exec}_{\textsf{a}-1}

    \textsf{input}_{\textsf{a}}\mexpandto \textsf{att}\mleft( \textsf{frame}_{\textsf{a}-1} \mright)%\\

    \textsf{frame}_{\textsf{a}} \mexpandto \begin{minipage}{0.7\columnwidth}%
        \begin{multline*}\ll \textsf{exec}_{\textsf{a}}; \\
            \ll \textbf{if }\textsf{exec}_{\textsf{a}}
                \textbf{ then }\textsf{output}_{\textsf{a}}
                \textbf{ else }\textsf{err}; \\
                \textsf{frame}_{\textsf{a}-1}\gg\gg
        \end{multline*}
    \end{minipage}
\end{mathpar}

Where $\ll \_; \_ \gg$, $\textbf{\textsc{if }}\_\textbf{\textsc{ then }}\_\textbf{\textsc{ else }}\_$ and $\dot\wedge$ are not use anywhere else.

==> 101-figures/101-logic-graph.tex <==
\pgfdeclarelayer{marrows}
\pgfdeclarelayer{mreferences}
\pgfsetlayers{marrows,main,mreferences}


\tikzset{reference/.style={draw,rectangle,fill=white, inner sep=2pt}}
\tikzset{mapping/.style={draw,thin,rectangle,color=black,fill=white,scale=0.8}}
\tikzset{logic/.style={draw,rectangle,rounded corners=3pt,fill=white}}
\tikzset{m>/.tip = {Stealth[scale=1.3]}}
\tikzset{<m/.tip = {Stealth[scale=1.3]}}

\begin{center}
\begin{tikzpicture}[scale=0.8]


    \node[logic] (BC) at (0, 0) {\BCLogic};
    \node[logic, above=of BC] (nS) {\begin{minipage}{2.3cm}\begin{center}
        Non-indexed \SymbLogic
    \end{center}\end{minipage}};
    \node[logic, above=of nS] (S){
        \SymbLogic};
    \node[logic, above=of S] (E) {\EvalLogic};

    \node[logic, right=of S] (Sq) {\msquirrel};

    \begin{pgfonlayer}{mreferences}
        \draw (BC.south east)  node[reference]{\scalebox{0.6}{\ref{sec:bc-logic}}};
        \draw (nS.south east)  node[reference]{\scalebox{0.6}{\ref{sec:ni-symbolic}}};
        \draw (S.south east)  node[reference]{\scalebox{0.6}{\ref{sec:unbound-protocol}}};
        \draw (E.south east)  node[reference]{\scalebox{0.6}{\ref{sec:evaluated}}};
        \draw (Sq.south east)  node[reference]{\scalebox{0.6}{\cite{baelde_cracking_2022}}};
    \end{pgfonlayer}

    \begin{pgfonlayer}{marrows}
        \draw[-m>] (S) to node[midway, mapping] {$\meval{\_}$} (E);
        \draw[->, line width=3pt, color=blue!10] (S) to[out=180, in=180,looseness=0.9] node[midway, mapping] {$\left( \_ \right)^\mathbb{T}$} (BC);

        \draw[-m>] (Sq) to[out=-90, in=0] (BC);
        \draw[<m-m>, dashed] (BC) to[out=180, in=180, looseness=1.2] node[midway, fill=white, inner sep=1.2pt] {\rotatebox{0}{\scalebox{0.6}{Prop.~\ref{prop:validity}}}} (E);
        \draw[-m>] (nS) to  node[midway, mapping] {$\left[ \_ \right]_\mathbb{E}$} (BC);
        \draw[-m>] (S) to node[midway, mapping] {$\left[ \_ \right]^\mathbb{I}$} (nS);

        \draw[<m-m>, dashed] (Sq) to[out=155, in=25] (S);
        \draw[<m-m>] (Sq) to[out=140, in=40] node[midway, fill=white, inner sep=1.2pt] {\scalebox{0.6}{\appref{sec:comp-w-squirrel}}} (S);

    \end{pgfonlayer}
\end{tikzpicture}
\end{center}

{\small\underline{Legend}:
\begin{itemize}
    \item %
\tikz[scale=0.7]{%
    \node[logic] (A) at (0, 0) {\tiny $L_1$};
    \node[logic] (B) at (1.5, 0) {\tiny $L_2$};
        \draw[-Stealth] (A) to  (B);
} denotes that we can transform terms from $L_1$ into terms of $L_2$. The optional label tells the notation used for such transformation.
    \item %
\tikz[scale=0.7]{%
    \node[logic] (A) at (0, 0) {\tiny $L_1$};
    \node[logic] (B) at (1.5, 0) {\tiny $L_2$};
        \draw[-{>[scale=0.8]}, line width=2pt, color=blue!10] (A) to  (B);
} denotes the composition of such transformations.
    \item %
\tikz[scale=0.7]{%
    \node[logic] (A) at (0, 0) {\tiny $L_1$};
    \node[logic] (B) at (1.5, 0) {\tiny $L_2$};
        \draw[Stealth-Stealth, dashed] (A) to  (B);
} denotes a noteworthy semantic relationship.
\end{itemize}}

==> 101-figures/euf-cma-formula.tex <==
\begin{equation}\label{eq:eufcma1}
    \forall m, \sigma, \mathsf{k}. \meval{\mverify{\sigma}{m}{\mathsf{k}}} \Rightarrow \left( \mathsf{k}\sqsubseteq_{\mhash{\_}{\bullet}} m, \sigma, \mathcal{P} \vee \exists u. \left( \mhash{u}{\mathsf{k}} \sqsubseteq m, \sigma \wedge \meval{u} = \meval{m} \right) \right)
\end{equation}

==> 101-figures/full-grammar.tex <==
\begin{align*}
    N \coloneqq&\quad      \mathsf{n}\!\left[ \vec \imath \right]
                        &\text{of sort \noncet}\\
    M \coloneqq&\quad      f\!\left( \vec t \right)
                \gsep \mathsf{input}(T)
                \gsep \bar N
                \gsep \mathsf{c}\!\left[ \vec \imath \right]\mat T \\
                &\gsep \textsf{find } \vec \imath \textsf{ such that } C \textsf{ then } M \textsf{ else } M'
                        &\text{of sort \msgt}\\
    C \coloneqq&\quad      f\!\left( \vec t \right)
                \gsep M \equiv M' \gsep i = i'
                \gsep \dot\exists \vec \imath, C,
                \gsep \dot\forall\vec \imath, C
                        &\text{of sort \condt}\\
    t \coloneqq&\quad      M
                \gsep C \\
    T \coloneqq&\quad      \mathsf{a}\!\left[ \vec \imath \right]
                \gsep \mathsf{pred}(T)
                        &\text{of sort \tpt} \\
    T_f \coloneqq&\quad    T = T'
                \gsep T < T'
                \gsep \mathsf{happens}\!\left( T \right)
                        &\text{of sort \boolt}\\
    S \coloneqq&\quad      t \sqsubseteq_* t'
                \gsep \dots
                        &\text{of sort \boolt}\\
    \phi \coloneqq&\quad   \meval{C}
                \gsep T_f \gsep S
                \gsep \top
                \gsep \bot
                \gsep \phi \diamond \phi'
                \gsep \neg\phi
                \gsep t = t' \\
                & \gsep \meval{M} = \meval{M'}
                \gsep \exists i. \phi
                \gsep \forall i. \phi
                \gsep \exists t. \phi
                \gsep \forall t. \phi
                        &\text{of sort \boolt}\\
    \diamond \coloneqq&\quad \vee
                \gsep \wedge
                \gsep \Rightarrow
\end{align*}

Where $f\in\mathcal{F}$, $\mathsf{n}\in \mathcal{N}$ %, $\mathsf{c}\in \mathcal{C}$
and $\mathsf{a}\in \mathcal{A}$.

==> 101-figures/full-semantics-figure.tex <==
Unchanged \msquirrel\ terms:
\begin{mathpar}
    \mintrhigh{\bar{\mathsf{n}}\!\left[ \vec \imath \right]} \mevalto \mathsf{n}\!\left[ \vec \imath \right]

    \mintrhigh{f\!\left( t_1,\dots, t_n \right)} \mevalto f\!\left( \mintrhigh{t_1},\dots, \mintrhigh{t_n} \right)

    \mintrhigh{\mathsf{input}(T)} \mevalto \mathsf{input}\mat\mintrhigh{T}

    \mintrhigh{\mathsf{c}\!\left[\vec \imath\right](T)} \mevalto \mathsf{c}\!\left[\vec \imath\right]\mat\mintrhigh{T}

    \mintrhigh{m \equiv m'} \mevalto \mintrhigh{m} \equiv \mintrhigh{m'}

    \mintrhigh{i = i'} \mevalto i = i'

    \mintrhigh{\dot\exists \vec \imath. c} \mevalto \bexists \imath. \mintrhigh{c}

    \mintrhigh{\dot\forall \vec \imath. c} \mevalto \bforall \imath. \mintrhigh{c}

    \mintrhigh{\mathsf{a}\!\left[ \vec \imath \right]} \mevalto \mathsf{a}\!\left[ \vec \imath \right]

    \mintrhigh{\mathsf{pred}(T)} \mevalto \mathsf{pred}(T)

    \mintrhigh{T = T'} \mevalto \mintrhigh{T} = \mintrhigh{T'}

    \mintrhigh{T < T'} \mevalto \mintrhigh{T < T'}

    \mintrhigh{\mathsf{happens}(T)} \mevalto \mathsf{happens}(T)

    \mintrhigh{\mfindst{\vec \imath}{c}{m}{m'}} \mevalto \mfindst{\vec \imath}{\mintrhigh{c}}{\mintrhigh{m}}{\mintrhigh{m'}}
\end{mathpar}

Preevaluated terms:
\begin{mathpar}
    \mintrhigh{\meval{C}} \mevalto \mintrhigh{C}

    \mintrhigh{\meval{M}=\meval{M'}} \mevalto \mintrhigh{M} \equiv \mintrhigh{M'}

    \mintrhigh{\top}\mevalto\btop

    \mintrhigh{\bot}\mevalto\bbot

    \mintrhigh{\neg\phi} \mevalto \begin{cases}
        \btop & \text{if $\mintrhigh{\phi}=\bbot$}\\
        \bbot & \text{if $\mintrhigh{\phi}=\btop$}\\
        \bneg\mintrhigh{\phi} & \text{otherwise}
    \end{cases}

    \mintrhigh{\phi\wedge\phi'} \mevalto \begin{cases}
        \bbot & \text{if $\mintrhigh{\phi}=\bbot$ or $\mintrhigh{\phi'}=\bbot$}\\
        \mintrhigh{\phi'} & \text{if $\mintrhigh{\phi}=\btop$}\\
        \mintrhigh{\phi} & \text{if $\mintrhigh{\phi'}=\btop$}\\
        \mintrhigh{\phi}\bwedge\mintrhigh{\phi'} & \text{otherwise}
    \end{cases}

    \mintrhigh{\phi \vee \phi'} \mevalto \mintrhigh{\neg \left( \neg \phi \wedge \neg \phi' \right)}

    \mintrhigh{\phi \Rightarrow \phi'} \mevalto \mintrhigh{\neg \phi \vee \phi'}

    \mintrhigh{\forall t. \phi} \mevalto \mintrhigh{\bigwedge_t \phi}

    \mintrhigh{\exists t. \phi} \mevalto \mintrhigh{\neg \left( \forall t. \neg\phi \right)}

    \mintrhigh{\exists i, \phi} \mevalto \begin{cases}
        \mintrhigh{\phi} & \text{if $\mintrhigh{\phi}=\bbot$ or $\mintrhigh{\phi}=\btop$}\\
        \bexists i, \mintrhigh{\phi} & \text{otherwise}
    \end{cases}

    \mintrhigh{\forall i, \phi} \mevalto \begin{cases}
        \mintrhigh{\phi} & \text{if $\mintrhigh{\phi}=\bbot$ or $\mintrhigh{\phi}=\btop$}\\
        \bforall i, \mintrhigh{\phi} & \text{otherwise}
    \end{cases}

    \mintrhigh{t=t'}\mevalto\begin{cases}
        \bar{\bigwedge}_{i\in v(t)}\,i=\sigma(i) & \text{if we can find a permutation $\sigma$ of the variables of $t$ st. $t\sigma = t'$}\\
        \bbot & \text{otherwise}
    \end{cases}

    \mintrhigh{t \sqsubseteq t'} \mevalto \mintrhigh{\bigvee_{\left( u, \vec \jmath, c \right)\in \msubtermset{1}{t'}} \exists \vec \jmath. t = u \wedge c}
\end{mathpar}

==> 101-figures/squirrel-semantics.tex <==
\begin{mathpar}
    \mintr{i} \mevalto \sigmI(i)

    \mintr{\mathsf{a}\!\left[ i_1,\dots,i_n \right]} \mevalto \mathsf{a}\!\left[ \mintr{i_1},\dots,\mintr{i_n} \right]

    % \mintr{\mathsf{pred}(T)} \mevalto \begin{cases}
    %     \mathsf{initr} & \text{if }\mintr{T}=\mathsf{init}\\
    %     \max_{\precT}\left\{ s \middle| s \precT \mintr{T}, s\in \domT \right\} & \text{if }\mintr{T}\in\domT\\
    %     \text{any step} & \text{otherwise}
    % \end{cases}
    \mintr{\mathsf{pred}(T)} \mevalto \mepred{\mintr{T}}

    \mintr{\mathsf{n}\!\left[ i_1,\dots,i_n \right]} \mevalto \mathsf{n}_{\mintr{i_1},\dots,\mintr{i_n}}

    \mintr{f\!\left( t_1,\dots,t_n \right)} \mevalto  f\!\left( \mintr{t_1},\dots, \mintr{t_n} \right)

    \mintr{\mathsf{c}\!\left[ i_1,\dots, i_n \right]\mat T} \mevalto \mintr{m}\text{ when $\mintr{T}=\mathsf{s}\left\{ \_ \right\}\left\{ \_ \right\}\left\{ \mathsf{c}\!\left[ \mintr{i_1},\dots,\mintr{i_n} \right]\leftarrow m,\dots \right\}$}

    \mintr{\mathsf{input}\mat T} \mevalto \mathsf{att}\!\left( \mathsf{frame}_{\mintr{T}} \right)

    \mintr{t\equiv t'} \mevalto \mathsf{EQ}\!\left( \mintr{t},\mintr{t'} \right)

    \mintr{i=i'}\mevalto\begin{cases}
        \mathsf{true}&\text{if }\mintr{i}=\mintr{i'}\\
        \mathsf{false}&\text{otherwise}
    \end{cases}

    \mintr{T=T'}\mevalto\begin{cases}
        \mathsf{true}&\text{if }\mintr{T}=\mintr{T'}\\
        \mathsf{false}&\text{otherwise}
    \end{cases}

    \mintr{T<T'}\mevalto\begin{cases}
        \mathsf{true}&\text{if }\mintr{T}\precT\mintr{T'}\\
        \mathsf{false}&\text{otherwise}
    \end{cases}

    \mintr{\mathsf{happens}(T)}\mevalto\begin{cases}
        \mathsf{true}&\text{if }\mintr{T}\in\domT\\
        \mathsf{false}&\text{otherwise}
    \end{cases}

    \mintr{\phi \bwedge \phi'} \mevalto
            \textsf{if }\mintr{\phi}\textsf{then }\mintr{\phi'}\textsf{ else }\mathsf{false}

    \mintr{\phi \bvee \phi'} \mevalto
            \textsf{if }\mintr{\phi}\textsf{then }\mathsf{true}\textsf{ else }\mintr{\phi'}

    \mintr{\bforall \vec \imath, c} \mevalto \mintr{\bar\bigwedge_{j}c^{\left\{ \vec \imath \mapsto \bm{\vec \imath}^{\domI}_j \right\}}}

    \mintr{\bexists \vec \imath, c} \mevalto \mintr{\bar\bigvee_{j}c^{\left\{ \vec \imath \mapsto \bm{\vec \imath}^{\domI}_j \right\}}}

    \mintr{\begin{minipage}{0.25\textwidth}%
        \vspace*{-5pt}\begin{multline*}
            \textsf{find }\vec\imath\textsf{ such that }c\\
            \textsf{then }m\textsf{ else }m'
        \end{multline*}
    \end{minipage}} \mevalto \begin{minipage}{0.6\textwidth}
        \vspace*{-5pt}\begin{multline*}
            \textsf{if }\mintr{c^{\left\{ \vec \imath \mapsto \bm{\vec \imath}^{\domI}_0 \right\}}}
                \textsf{ then }\mintr{m^{\left\{ \vec \imath \mapsto \bm{\vec \imath}^{\domI}_0 \right\}}}\textsf{ else }\dots\\
            \textsf{if }\mintr{c^{\left\{ \vec \imath \mapsto \bm{\vec \imath}^{\domI}_n \right\}}}
                \textsf{ then }\mintr{m^{\left\{ \vec \imath \mapsto \bm{\vec \imath}^{\domI}_n \right\}}}\textsf{ else }\mintr{m'}
        \end{multline*}
    \end{minipage}
\end{mathpar}
For simplicity of the notations, we assume w.l.o.g. in this figure that all steps assign to all memory cells. Any unassigned cell $\mathsf{c}$ at step $\mathsf{s}$ can be assigned $\mathsf{c}\mat \mathsf{pred}(\mathsf{s})$.

\begin{align*}
    \mathsf{cond}_\mathsf{a}&=c &\text{when $\mathsf{a}=\mathsf{a}\left\{ m \right\}\left\{ c \right\}\left\{ \dots \right\}$}\\
    \mathsf{msg}_\mathsf{a}&=m &\text{when $\mathsf{a}=\mathsf{a}\left\{ m \right\}\left\{ c \right\}\left\{ \dots \right\}$}\\
    \mathsf{exec}_\mathsf{init}^\mathbb{T}&=\mathsf{cond}_\mathsf{init}\\
    \mathsf{frame}_\mathsf{init}^\mathbb{T}&=\mathsf{msg}_\mathsf{init}\\
    \mathsf{exec}_\mathsf{a}^\mathbb{T}&=\mathsf{cond}_\mathsf{a}\wedge\mathsf{exec}_{\mepred[\mathbb{T}]{\mathsf{a}}}\\
    \mathsf{frame}_\mathsf{a}^\mathbb{T}&=\textsf{if }\mathsf{exec}_\mathsf{a}^\mathbb{T}\textsf{ then }\left(\mathsf{cond}_\mathsf{a}, \mathsf{msg}_\mathsf{a}, \mathsf{frame}_{\mepred[\mathbb{T}]{\mathsf{a}}}^\mathbb{T}\right)\textsf{ else }\varnothing
\end{align*}

==> 101-figures/subterm-set/order.tex <==

 
\begin{mathpar}
    T_0\triangleleft u \coloneqq \overline{\bigvee}_{\left( \mmacro{m}{T}, \vec\imath \right)\in \msti{u}} \bexists \vec\imath. T_0 \blacktriangleleft \mmacro{m}{T}

T_0 \blacktriangleleft \mmacro{m}{T} \coloneqq \begin{cases}
    T_0 < T &\text{if $\mathsf{m}$ is $\mathsf{input}$}\\
    T_0 \leq T &\text{otherwise}
\end{cases}
\end{mathpar}
 restore

==> 101-figures/subterm-set/sti.tex <==
 
\begin{mathpar}
    \msti{\mathfrak{f}\left( t_1,\dots, t_k \right)} \coloneqq \left\{ (\mathfrak{f}\left( t_1,\dots, t_k \right), \varnothing) \right\} \cup\bigcup\nolimits_{i=1}^k \msti{t_i} 

    \msti{\mmacro{m}{T}} \coloneqq \left\{ \left( \mmacro{m}{T}, \varnothing \right) \right\}

    \msti{\mathsf{n}\left[ \vec \imath \right]} \coloneqq \left\{ \left( \mathsf{n}\left[ \vec \imath \right], \varnothing \right) \right\}

    \msti{\mathfrak{Q}\vec x. u_1,\dots, u_k} \coloneqq \left\{ (\mathfrak{Q}\vec x. u_1,\dots, u_k, \varnothing) \right\} \cup\bigcup\nolimits_{i=1}^k \left\{ \left( v, \vec y \uplus \vec x \right) \middle| \left( v, \vec y \right) \msti{t_i} \right\} 
\end{mathpar}
where $\mathfrak{f}$ stands for $f, \equiv,\allowbreak \btop,\allowbreak \bbot,\allowbreak \bwedge,\allowbreak \bvee,\allowbreak \bneg$ or $\textsc{if }\_\allowbreak\textsc{ then }\_\allowbreak\textsc{ else }\_$ and $\mathfrak{Q}$ for $\bexists,\allowbreak \bforall$ or $\mfindst{\_\allowbreak}{\_\allowbreak}{\_\allowbreak}{\_}$.
 restore

==> 101-figures/subtermset.tex <==
\begin{mathpar}
    \msubtermset{l}{f\!\left( t_1,\dots, t_n \right)}=\left\{ (\varnothing, \top, f\!\left( t_1,\dots, t_n \right)) \right\} \cup\bigcup_{i=1}^n\msubtermset{l}{t_i}

    \msubtermset{l}{\bar{\mathsf{n}}} = \left\{ \left(\varnothing, \top, \bar{\mathsf{n}} \right) \right\}

    \msubtermset{l}{m\equiv m'} = \msubtermset{l}{m\equiv m'}\cup\msubtermset{l}{m}\cup\msubtermset{l}{m'}

    \msubtermset{l}{i=i'}=\left\{ (\varnothing, \top, i=i') \right\}

    \msubtermset{l}{\dot\exists \vec \imath. c} = \left\{ (\varnothing, \top, \dot\exists \vec \imath. c) \right\} \cup \left\{ (\vec\imath \cup \vec\jmath,\phi, t) \middle| (\vec\jmath, \phi, t)\in \msubtermset{l}{c} \right\}

    \msubtermset{l}{\dot\forall \vec \imath. c} = \left\{ (\varnothing, \top, \dot\forall \vec \imath. c) \right\} \cup \left\{ (\vec\imath \cup \vec\jmath,\phi, t) \middle| (\vec\jmath, \phi, t)\in \msubtermset{l}{c} \right\}

    \msubtermset{l}{\mfindst{\vec\imath}{c}{m}{m'}} =
    \begin{minipage}{0.55\textwidth}
        \vspace*{-5pt}\begin{multline*}
            \left\{ (\varnothing, \top, \mfindst{\vec\imath}{c}{m}{m'}) \right\} \\
            \cup \left\{ (\vec\imath \cup \vec\jmath,\phi, t) \middle| (\vec\jmath, \phi, t)\in \msubtermset{l}{c, m} \right\} \\
            \cup \msubtermset{l}{m'}
        \end{multline*}
    \end{minipage}

    \msubtermset{h}{\mathsf{c}\!\left[ \vec \imath \right]\mat \tau} = % = \bigcup_{\mathsf{a}\!\left[ \vec\jmath \right]\left\{ \dots \right\}\left\{ \dots \right\}\left\{ \mathsf{c}\!\left[ \vec l \right] \leftarrow m\right\}} \left\{ \left(\vec\jmath\cup\vec{k}, \vec\imath=\vec l \wedge \tau \leq  \mathsf{a}\!\left[ \vec\jmath \right] \wedge c, m' \right) \middle| \left(\vec k, c, m'\right) \in \msubtermset{h}{m} \right\}
    \begin{minipage}{0.7\textwidth}
        \vspace*{-5pt}\begin{multline*}
            \bigcup_{\mathsf{a}\!\left[ \vec\jmath \right]\left\{ \dots \right\}\left\{ \dots \right\}\left\{ \mathsf{c}\!\left[ \vec l \right] \leftarrow m\right\}} \left\{ \left(\vec\jmath\cup\vec{k}, \vec\imath=\vec l \wedge \tau \leq  \mathsf{a}\!\left[ \vec\jmath \right] \wedge c, m' \right) \middle| \left(\vec k, c, m'\right) \in \msubtermset{h}{m} \right\}\\
            \cup \left\{ (\varnothing, \top, \mathsf{c}\!\left[ \vec \imath \right]\mat \tau) \right\}
        \end{multline*}
    \end{minipage}

    \msubtermset{1}{\minput{\tau}} = % \left\{ \varnothing, \top,  \mathsf{input}(\tau)\right\}\cup\bigcup_{\mathsf{a}[\vec \imath]\in \mathcal{P}}\left\{ (\vec \imath\cup \vec \jmath, \mathsf{a}\!\left[ \vec \imath \right] < \tau \wedge c, t') \middle| (\vec \jmath, c, t')\in \msubtermset{2}{\mathsf{msg}(\mathsf{a}), \mathsf{cond}(\mathsf{a})} \right\}
    \begin{minipage}{0.7\textwidth}
        \vspace*{-5pt}\begin{multline*}
            \bigcup_{\mathsf{a}[\vec \imath]\in \mathcal{P}}\left\{ (\vec \imath\cup \vec \jmath, \mathsf{a}\!\left[ \vec \imath \right] < \tau \wedge c, t') \middle| (\vec \jmath, c, t')\in \msubtermset{2}{\mmsg{\mathsf{a}}, \mcond{\mathsf{a}}} \right\}\\
            \cup\left\{ \varnothing, \top,  \minput{\tau}\right\}
        \end{multline*}
    \end{minipage}

    \msubtermset{2}{\minput{\tau}} = \left\{ \varnothing, \top,  \minput{\tau}\right\}
\end{mathpar}
